A Model Is Not Built By A Single Prompt: LLM-Based Domain Modeling With Question Decomposition

Domain modeling, a crucial part of model-driven engineering, demands extensive domain knowledge and experience from engineers. When the system description is highly complicated, the modeling task can become particularly challenging and time-consuming. Large language Models(LLMs) can assist by automatically generating an initial object model from the system description. Although LLMs have demonstrated remarkable code-generation ability, they still struggle with model-generation using a single prompt. In real-world domain modeling, engineers usually decompose complex tasks into easily solvable sub-tasks, significantly controlling complexity and enhancing model quality. Inspired by this, we propose an LLM-based domain modeling approach via question decomposition, similar to developer's modeling process. Following conventional modeling guidelines, we divide the model generation task into several sub-tasks, i.e., class generation, association and aggregation generation, and inheritance generation. For each sub-task, we carefully design the prompt by choosing more efficient query words and providing essential modeling knowledge to unlock the modeling potential of LLMs. To sum up all the sub-tasks solutions, we implemente a proof-of-object tool integrated into the standard Ecore editor that asks LLMs to generate an object model from the system description. We evaluate our approach with 20 systems from different application domains. The preliminary results show that our approach outperforms the single-prompt-based prompt by improving recall values and F1 scores in most systems for modeling the classes, attributes, and relationships.

==> section/discussion.tex <==
\section{Discussion and future work }\label{sec:discussion}
In this section, we discuss some limitations of this work and present some potential directions for future work.
% \textbf{limitations and future works: }
\begin{itemize}
    \item There is still room for improvement in our approach. Beacuse our approach cannot predict the names of associations (aggregations), and the overall F1 score should be further improved before it can be put into practice. We plan to refine our approach, especially by adopting more advanced prompt engineering techniques.
    \item Although the tool is an LLM-based, fully automated domain modeling tool, there are still some gaps between the prototype tool and the actual software development scenarios. we will enhance our prototype tool in functionality and usability, and will contribute it to the MDE community. But we allow humans as the last link to verify the modeling results, helping to enhance the usefulness of our approach in real-world application scenarios.
    \item we plan to improve our evaluation by testing more systems on different LLMs, and explore the potential for fine-tuning LLMs for model generation.
\end{itemize}

